Descending Price Auctions with Bounded Number of Price Levels and Batched Prophet Inequality

We consider descending price auctions for selling $m$ units of a good to unit demand i.i.d. buyers where there is an exogenous bound of $k$ on the number of price levels the auction clock can take. The auctioneer's problem is to choose price levels $p_1 > p_2 > \cdots > p_{k}$ for the auction clock such that auction expected revenue is maximized. The prices levels are announced prior to the auction. We reduce this problem to a new variant of prophet inequality, which we call \emph{batched prophet inequality}, where a decision-maker chooses $k$ (decreasing) thresholds and then sequentially collects rewards (up to $m$) that are above the thresholds with ties broken uniformly at random. For the special case of $m=1$ (i.e., selling a single item), we show that the resulting descending auction with $k$ price levels achieves $1- 1/e^k$ of the unrestricted (without the bound of $k$) optimal revenue. That means a descending auction with just 4 price levels can achieve more than 98\% of the optimal revenue. We then extend our results for $m>1$ and provide a closed-form bound on the competitive ratio of our auction as a function of the number of units $m$ and the number of price levels $k$.

==> tex/macros.tex <==
\usepackage{eurosym}
\usepackage{graphicx,amsmath,amsfonts}
\usepackage{setspace}
\usepackage{amssymb}
\usepackage{dsfont}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{ifthen}
\usepackage{mathtools}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{color}
\usepackage{framed}
\usepackage[margin=1in]{geometry}
\usepackage[authoryear,round]{natbib}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorlinks=true, urlcolor=Mahogany, linkcolor=Mahogany, citecolor=Mahogany]{hyperref}
\usepackage{fp}
\usepackage[abspage,user,savepos]{zref}
\usepackage[capitalize]{cleveref}
\usepackage{amsthm}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{palatino}
\usepackage{cuted,balance}
\usepackage{cleveref}

\setcounter{MaxMatrixCols}{10}
%TCIDATA{OutputFilter=LATEX.DLL}
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{Codepage=65001}
%TCIDATA{<META NAME="SaveForMode" CONTENT="1">}
%TCIDATA{BibliographyScheme=BibTeX}
%TCIDATA{LastRevised=Wednesday, August 05, 2020 22:46:20}
%TCIDATA{<META NAME="GraphicsSave" CONTENT="32">}
\usepackage[ruled]{algorithm2e} 
\renewcommand{\algorithmcfname}{Mechanism}


\newcommand{\BREAKCOL}{&&&}
\newtheorem*{thma}{Theorem}
\newtheorem{Lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{alg}{Algorithm}
\newcommand{\propositionautorefname}{Proposition}
\renewcommand{\equationautorefname}{Eq.}
\renewcommand{\figureautorefname}{Fig.}
\newcommand{\exampleautorefname}{Example}
\newcommand{\assumptionautorefname}{Assumption}
\newcommand{\corollaryautorefname}{Corollary}
\newcommand{\Lemmaautorefname}{Lemma}

\newcommand{\argmax}{\operatorname{arg\ max}}
\newcommand{\argmaxone}{\operatorname{arg^{\dag} max}}
\newcommand{\argmin}{\operatorname{arg\ min}}


\newcommand{\comment}[1]{\noindent\fbox{\textbf{\color{red}Comment: #1}} \index{COMMENT}}
\let\originaleqref\eqref
\renewcommand{\eqref}{\originaleqref}
\vskip 2pc \onehalfspace


==> tex/macros_EC.tex <==
\usepackage{eurosym}
\usepackage{graphicx,amsmath,amsfonts}
\usepackage{setspace}
%\usepackage{amssymb}
\usepackage{dsfont}
\usepackage{amsmath}
\usepackage{ifthen}
\usepackage{mathtools}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{color}
\usepackage{framed}
\usepackage{natbib}
\usepackage{csquotes}

\makeatletter
%Take the original environment definition and change the leftmargin to 1cm
\renewenvironment*{displayquote}
  {\begingroup\setlength{\leftmargini}{0.5cm}\csq@getcargs{\csq@bdquote{}{}}}
  {\csq@edquote\endgroup}
\makeatother
%\usepackage[dvipsnames]{xcolor}
%
\usepackage{fp}
\usepackage[abspage,user,savepos]{zref}
\usepackage[capitalize]{cleveref}
\usepackage{amsthm}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{palatino}
\usepackage{cuted,balance}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\setcounter{MaxMatrixCols}{10}

\newcommand{\BREAKCOL}{&&&}
\newtheorem*{thma}{Theorem}
\newtheorem{Lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{alg}{Algorithm}
%\usepackage{amsmath,bm}


\newcommand{\propositionautorefname}{Proposition}
\renewcommand{\equationautorefname}{Eq.}
\renewcommand{\figureautorefname}{Fig.}
\newcommand{\exampleautorefname}{Example}
\newcommand{\assumptionautorefname}{Assumption}
\newcommand{\corollaryautorefname}{Corollary}
\newcommand{\Lemmaautorefname}{Lemma}

% \newcommand{\argmax}{\operatorname{arg\ max}}
% \newcommand{\argmaxone}{\operatorname{arg^{\dag} max}}
% \newcommand{\argmin}{\operatorname{arg\ min}}






%%%

%%%

\let\originaleqref\eqref
\renewcommand{\eqref}{\originaleqref}

%\vskip 2pc \onehalfspace


\usepackage{acm-ec-22}

\usepackage{booktabs} % For formal tables


\usepackage[ruled]{algorithm2e} % For algorithms
\renewcommand{\algorithmcfname}{ALGORITHM}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}

\newcommand{\rad}[1]{{\color{red}[\textbf{Rad:}~#1]}}
\newcommand{\ali}[1]{{\color{blue}[\textbf{Ali:}~#1]}}
\newcommand{\azar}[1]{{\color{purple}[\textbf{Azar:}~#1]}}





%###############################
\newcommand{\buyerset}{\mathcal{N}}
\newcommand{\vbf}{\mathbf{v}}
\newcommand{\buyerCDF}{G}
\newcommand{\buyerPDF}{g}
\newcommand{\virtualV}{\phi_{\buyerCDF}}
\newcommand{\ironvirtualV}{\bar{\phi}_{\buyerCDF}}
\newcommand{\levelNum}{k}
\newcommand{\pbf}{\mathbf{p}}
\newcommand{\bidset}{\mathcal{P}}
\newcommand{\eqbid}{b^*}
\newcommand{\rev}[2]{\textsc{Rev-ALG}_{\buyerCDF}\left(#1,#2\right)}
\newcommand{\opt}[1]{\textsc{Rev-OPT}_{\buyerCDF}\left(#1\right)}
\newcommand{\PriceThresh}{\Gamma_{\buyerCDF}}
\newcommand{\ThreshPrice}{\PriceThresh^{-1}}
\newcommand{\maxV}{\textrm{OPT}}
\newcommand{\algT}{\textrm{ALG}}
